CoMT: A Novel Benchmark for Chain of Multi-modal Thought on Large Vision-Language Models

Large Vision-Language Models (LVLMs) have recently demonstrated amazing success in multi-modal tasks, including advancements in Multi-modal Chain-of-Thought (MCoT) reasoning. Despite these successes, current benchmarks still follow a traditional paradigm with multi-modal input and text-modal output, which leads to significant drawbacks such as missing visual operations and vague expressions. Motivated by this, we introduce a novel Chain of Multi-modal Thought (CoMT) benchmark to address these limitations. Different from the traditional MCoT benchmark, CoMT requires both multi-modal input and multi-modal reasoning output, aiming to mimic human-like reasoning that inherently integrates visual operation. Specifically, CoMT consists of four categories: (1) Visual Creation, (2) Visual Deletion, (3) Visual Update, and (4) Visual Selection to comprehensively explore complex visual operations and concise expression in real scenarios. We evaluate various LVLMs and strategies on CoMT, revealing some key insights into the capabilities and limitations of the current approaches. We hope that CoMT can inspire more research on introducing multi-modal generation into the reasoning process.

==> sections/checklist.tex <==
\paragraph{This paper:}
\begin{itemize}
	\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) {\bf NA}
	\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) {\bf yes}
	\item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes/no) {\bf yes}
\end{itemize}

\paragraph{Does this paper make theoretical contributions? (yes/no)} {\bf yes}

If yes, please complete the list below.
\begin{itemize}
	\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no) {\bf yes}
	\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no) {\bf yes}
	\item Proofs of all novel claims are included. (yes/partial/no) {\bf yes}
	\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no) {\bf yes}
	\item Appropriate citations to theoretical tools used are given. (yes/partial/no) {\bf yes}
	\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA) {\bf NA}
	\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA) {\bf NA}
\end{itemize}

\paragraph{Does this paper rely on one or more datasets? (yes/no)} {\bf yes}

If yes, please complete the list below.
\begin{itemize}
	\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) {\bf yes}
	\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) {\bf no}
	\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) {\bf yes}
	\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA) {\bf yes}
	\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA) {\bf yes}
	\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) {\bf NA}
\end{itemize}

\paragraph{Does this paper include computational experiments? (yes/no)} {\bf yes}

If yes, please complete the list below.
\begin{itemize}
	\item Any code required for pre-processing data is included in the appendix. (yes/partial/no) {\bf no}
	\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) {\bf no}
	\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) {\bf yes}
	\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. (yes/partial/no) {\bf yes}
	\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) {\bf NA}
	\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) {\bf partial}
	\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) {\bf yes}
	\item This paper states the number of algorithm runs used to compute each reported result. (yes/no) {\bf yes}
	\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) {\bf yes}
	\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) {\bf yes}
	\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA) {\bf partial}
	\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) {\bf NA}
\end{itemize}

==> sections/potential_impact.tex <==
\section*{Potential Impact}
%We propose a novel chain of multi-modal thought (\datasetname{}) benchmark, aiming to evaluate and enhance the ability of VLLMs with multi-modal reasoning process.
%However, due to time and cost constraints, we currently evaluate the performance of VLLMs solely through prompting methods. Investigating how to endow the models with effective multi-modal reasoning capabilities is an important area for future research. 
%%We plan to examine the potential improvements that supervised fine-tuning on \datasetname{} can offer in future studies.
%Additionally, due to the inherent subjectivity of manual annotations, potential biases may be introduced. During the annotation process, we strive to mitigate these biases by focusing on relatively objective problems. 

Chain-of-Thought (CoT) is an essential method to induce large language models to perform step-by-step reasoning. As an extension, multi-modal CoT (MCoT) significantly enhances the reasoning performance of vision large language models (VLLMs) in handling multi-modal tasks. However, current MCoT benchmarks still follow a paradigm of multi-modal input and text-modal output, which leads to issues of missing visual expression and vague expression, limiting the performance of VLLMs. Our work focuses on introducing a benchmark (\datasetname{}) that requires both multi-modal input and multi-modal reasoning output, encompassing four types of visual operations. This benchmark aims to enhance VLLMs' ability to integrate visual expression and concise expression into rationale and can potentially promote the development of VLLMs in text-visual modality alignment.
